Adaptive Network Response to Line Failures in Power Systems

Transmission line failures in power systems propagate and cascade non-locally. In this work, we propose an adaptive control strategy that offers strong guarantees in both the mitigation and localization of line failures. Specifically, we leverage the properties of network bridge-block decomposition and a frequency regulation method called the unified control. If the balancing areas over which the unified control operates coincide with the bridge-blocks of the network, the proposed strategy drives the post-contingency system to a steady state where the impact of initial line outages is localized within the areas where they occurred whenever possible, stopping the cascading process. When the initial line outages cannot be localized, the proposed control strategy provides a configurable design that progressively involves and coordinates more balancing areas. We compare the proposed control strategy with the classical Automatic Generation Control (AGC) on the IEEE 118-bus and 2736-bus test networks. Simulation results show that our strategy greatly improves overall reliability in terms of the N-k security standard, and localizes the impact of initial failures in the majority of the simulated contingencies. Moreover, the proposed framework incurs significantly less load loss, if any, compared to AGC, in all our case studies.

==> LoadSheddingRef.tex <==

Load shedding to mitigate cascading failure has been studied in the literature, e.g., 
using reinforcement learning \cite{Jung2002},
by shedding only the interruptible part of each load \cite{Faranda2007},
adaptively using affine control based on observed state \cite{bienstock2011control},
formulated as a DCOPF problem \cite{Pahwa2013}, or 
by treating the cascading process as a discrete-time optimal control problem \cite{BaSavla2019}.
DC power flow model is used in \cite{bienstock2011control, Pahwa2013, BaSavla2019} as in this paper.
Unlike these papers, we do not propose separate load shedding at the slow (power flow) timescale.
Instead, load (and generation) control is performed as part of frequency regulation during both
normal operation and contingency.

==> acknowledgement.tex <==
This work has been supported by Resnick Fellowship, Linde Institute Research Award, NWO Rubicon grant 680.50.1529., NSF grants through PFI:AIR-TT award 1602119, EPCN 1619352, CNS 1545096, CCF 1637598, ECCS 1619352, CNS 1518941, CPS 154471, AitF 1637598, ARPA-E grant through award DE-AR0000699 (NODES) and GRID DATA, DTRA through grant HDTRA 1-15-1-0003 and Skoltech through collaboration agreement 1075-MRA.

==> basic.tex <==
We have introduced two distinct partitions of a power network so far: the tree-partition $\calP^{\text{tree}}$ in Part I and the control area partition $\calP^{\text{UC}}$ in Section~\ref{section:preliminaries}. In general, $\calP^{\text{tree}}$ and $\calP^{\text{UC}}$ can be different. However, when they do coincide, the underlying power grid inherits analytical properties from both tree-partition and UC, making the system particularly robust against failures. Our proposed control strategy leverages precisely this connection, as we present in more detail in Section \ref{section:control_strategy}.

To create a tree-partition whose regions coincide the control areas over which UC operates, some tie-lines of $\calP^{\text{UC}}$ might be selected to switch off. Such selection can be systematically optimized under certain objectives. Interested reader are referred to \cite{zocca2019spectral} for more details. We henceforth assume that $\calP^{\text{tree}}=\calP^{\text{UC}}$. Under this assumption, the bridges and the tie-lines of the power network $\calG$ also coincide.%, and we use these two terms interchangeably in the sequel.

\begin{defn}
Given a cascading failure process described by $\calB(\n)$, with $\n\in\set{1,2, \ldots, N}$, the set $\calB(1)$ is said to be its \textbf{\emph{initial failure}}.
\end{defn}

In a power system, it is reasonable to expect that different initial failures can have different levels of impact on the rest of the network. For instance, the disconnection of a single solar panel from the grid is unlikely to cause any disruption to the system operation, while the failure of a transmission line that connects a major generator to the grid may incur significant load shedding. We thus need to distinguish different types of failures and ensure that the proposed control scheme reacts accordingly.

\begin{defn} \label{def:critical}
An initial failure $\calB(1)$ is said to be \textbf{\emph{critical}} if the UC optimization \eqref{eqn:uc_olc} is infeasible over $\calG(1):=(\calN, \calE\bs\calB(1))$, or \textbf{\emph{non-critical}} otherwise.
\end{defn}

To formally state our localization result, we define the following concept to clarify the precise meaning of a region being ``local'' with respect to an initial failure.

\begin{defn}
Given an initial failure $\calB(1)$, we say that a tree-partition region $\calN_l$ is \textbf{\emph{associated}} with $\calB(1)$ if there exists an edge $e=(i,j)\in\calB(1)$ such that either $i\in\calN_l$ or $j\in\calN_l$.
\end{defn}

As we discuss in Section \ref{section:control_strategy}, our control strategy provides strong guarantees in mitigation and localization for both non-critical and critical failures, in a way that only the operation of the associated regions are adjusted whenever possible.

==> concerns.tex <==
\todo{economic and environmental aspect, turbine governor model, voltage angle stability}

==> laplace_solvability_proof.tex <==
It is well-known (see \cite{guo2017monotonicity} for instance) that the Laplacian matrix $L:=CBC^T$ of a connected graph $\calG=(\calN,\calE)$ has rank $\abs{\calN} - 1$, and $Lx=b$ is solvable if and only if $\bff{1}^Tb=0$, where $\bff{1}$ is the vector with proper dimension that consists of ones. Moreover, the kernel of $L$ is given by $\spann(\bff{1})$.

If $\calN_1$ is the only area in $\calP$, then $b=0$ since $b_j=0$ for all $j\in\calN_1$. We thus know the solution space to $Lx=b$ is exactly the kernel of $L$, and the desired result holds.

If $\calN_1$ is not the only area in $\calP$, we can then find a node that does not belong to $\calN_1$, say node $z$. 
Without loss of generality, assume the node $z\in\calN_k$.
Consider a solution $x$ to $Lx=b$. Since the kernel of $L$ is $\spann(\bff{1})$,  we can without loss of generality assume the last component of $x$ is $0$. Let $\ol{L}$ be the submatrix of $L$ obtained by removing its last row and last column, and similarly let $\ol{x}$ and $\ol{b}$ be the vectors obtained by removing the last component of $x$ and $b$, respectively. Then $\ol{L}$ is invertible (since it is a principal submatrix, see \cite{guo2017monotonicity}), and we have
$$
\ol{L}\ol{x}=\ol{b}.
$$
Denote the matrix obtained by deleting the $l$-th row and $i$-th column of $\ol{L}$ by $\ol{L}^{li}$, then Proposition V.2 of \cite{guo2017monotonicity} shows that
\begin{equation}\label{eqn:graph_interpretation}
\det\paren{\ol{L}^{li}}=(-1)^{l+i}\sum_{E\in\calT(\set{l,i}, \set{z})}\chi(E)
\end{equation}
where $\chi(E)=\prod_{e\in E} B_e$ and $\calT(\set{l,i}, \set{z})$ is the set of spanning forests of $\calG$ that consists of exactly two trees containing $\set{l,i}$ and $\set{z}$ respectively. We refer the readers to \cite{guo2017monotonicity} for detailed discussion on these notations.

To state some useful results derived from  \eqref{eqn:graph_interpretation}, we introduce the following definition of directly connected areas.
\begin{defn}
For tree-partition areas $\calP=\set{\calN_1,\calN_2,\cdots, \calN_k}$ of $\calG$, we say $\calN_v$ and $\calN_w$ are \emph{\textbf{directly connected without $\calN_l$}} if the path from $\calN_v$ to $\calN_w$ in $\calG_\calP$ does not contain $\calN_l$. 
\end{defn}
The path from $\calN_v$ to $\calN_w$ in the above definition is unique since the areas are connected in a tree structure. 
\begin{lemma}\label{lemma:not_directly_connected}
Assume $\calN_2$ and $\calN_k$ are not directly connected without $\calN_1$. If $l_1,l_2\in\calN_2$ and $i\in \ol{\calN}_1$, then
$$
\calT(\set{l_1,i}, \set{z}) = \calT(\set{l_2,i},\set{z}).
$$
\end{lemma}
\begin{proof}
The path from $\calN_1$ to $\calN_k$ in $\calG_\calP$ contains a bridge in $\calG$ that incidents to $\calN_1$. Denote this bridge as $\tilde{e}$ and let $w$ be the endpoint of $\tilde{e}$ that is not in $\calN_1$. Then $w$ is a cut vertex that any path from $\ol{\calN}_1$ to $\calN_2$ must contain.

Since $\calN_2$ and $\calN_k$ are not directly connected without $\calN_1$, the path from $\calN_2$ to $\calN_k$ in $\calG_\calP$ passes through $\calN_1$. In other words, any path in $\calG$ from $\calN_2$ to $\calN_k$ must pass throughs a certain node in $\calN_1$, and thus contains a sub-path from $\calN_1$ to $\calN_k$. This implies that $w$ is contained in any path in $\calG$ from $\calN_2$ to $\calN_k$.

Note that any tree containing $i\in\ol{\calN}_1$ and $l_1\in\calN_2$ induces a path from $\ol{\calN}_1$ to $\calN_2$ and thus contains $w$. Further, any tree containing $l_2\in\calN_2$ and $z\in\calN_k$ induces a path from $\calN_2$ to $\calN_k$, and thus also contains $w$. As a result, these two types of trees always share a common node $w$ and cannot be disjoint:
$$
\calT(\set{l_1,i}, \set{l_2,z})= \emptyset
$$
Similarly $\calT(\set{l_2,i}, \set{l_1,z})= \emptyset$. Therefore
\begin{IEEEeqnarray*}{rCl}
&&\calT(\set{l_1,i}, \set{z})\\
&=&\calT(\set{l_1, l_2, i}, \set{z})\sqcup\calT(\set{l_1,i}, \set{l_2, z})\\
&=&\calT(\set{l_1, l_2, i}, \set{z})\sqcup\calT(\set{l_2,i}, \set{l_1, z})\\
&=&\calT(\set{l_2,i}, \set{z})
\end{IEEEeqnarray*}
where $\sqcup$ means disjoint union. The desired result then follows.
\end{proof}
\begin{lemma}\label{lemma:directly_connected}
Assume $\calN_2$ and $\calN_k$ are directly connected without $\calN_1$. If $l\in\calN_2$ and $i_1, i_2 \in\ol{\calN_1}$, then
$$
\calT(\set{l,i_1}, \set{z}) = \calT(\set{l,i_2},\set{z}).
$$
\end{lemma}
\begin{proof}
The path from $\calN_1$ to $\calN_k$  (denoted as $P_1$) contains one bridge in $\calG$ that incidents to $\calN_1$. Denote this bridge $\tilde{e}$ and let $w$ be the endpoint of $\tilde{e}$ that does not belong to $\calN_1$. Then $w$ is a cutting node that any path in $\calG$ from $\ol{\calN}_1$ to $\calN_k$ must pass through.

We claim that if $\calN_2$ and $\calN_k$ are directly conncted without $\calN_1$, then any path from $\ol{\calN}_1$ to $\calN_2$ in $\calG$ must also contain $w$. Indeed, suppose not, then the path from $\calN_1$ to $\calN_2$ (denoted as $P_2$) contains a bridge in $\calG$ that incidents to $\calN_1$, and this bridge is different from $\tilde{e}$. If $P_1$ and $P_2$ do not have any common super nodes, then concatenating the two paths induces a path from $\calN_2$ to $\calN_k$ that passes through $\calN_1$. In other words, the path from $\calN_2$ to $\calN_k$ passes through $\calN_1$, contradicting the assumption that $\calN_2$ and $\calN_k$ are directly connected without $\calN_1$. Therefore, $P_1$ and $P_2$ share a common 
area, say $\tilde{\calN}$. However, $P_1$ and $P_2$ induce two different sub-paths from $\calN_1$ to $\tilde{\calN}$, contracting the assumption that the areas forms a tree. We thus have proved the claim.
 
Finally, note that any tree containing $i_1\in\ol{\calN}_1$ and $l\in\calN_2$ induces a path from $\ol{\calN}_1$ to $\calN_2$ and thus contains $w$. Further, any tree containing $i_2\in\ol{\calN}_1$ and $z\in\calN_k$ induces a path from $\ol{\calN}_1$ to $\calN_k$ and thus contains $w$. Therefore these two types of trees always share a common node $w$ and cannot be disjoint:
$$
\calT(\set{l,i_1},\set{i_2, z})=\emptyset
$$
Similarly $=\calT(\set{l,i_2},\set{i_1, z})=\emptyset$. As a result,
\begin{IEEEeqnarray*}{rCl}
&&\calT(\set{l,i_1}, \set{z})\\
&=&\calT(\set{l,i_1, i_2}, \set{z})\sqcup\calT(\set{l,i_1}, \set{i_2, z})\\
&=&\calT(\set{l,i_1, i_2}, \set{z})\\
&=&\calT(\set{l,i_1, i_2}, \set{z})\sqcup\calT(\set{l,i_2}, \set{i_1, z})\\
&=&\calT(\set{l,i_2}, \set{z})
\end{IEEEeqnarray*}
\end{proof}
\noindent Since $b_k=\ol{b}_k=0$ for all $k\in\calN_1$, by Cramer's rule,
\begin{equation}\label{eqn:component_inversion}
x_i=\ol{x}_i=\frac{\sum_{l\notin \calN_1}(-1)^{l+i}b_k\det\paren{\ol{L}^{li}}}{\det\paren{\ol{L}}}, \text{ for all $i$.}
\end{equation}
% for all $i$.

Let $\calP_1$ be set of the areas in $\calP$ that are directly connected to $\calN_k$ without $\calN_1$ and let $\calP_2$ be the remaining areas. For an area $\calN_l\in\calP_1$, let
$$
\chi(\calN_l):=\sum_{E\in\calT(\set{\tilde{l},i},\set{z})}\chi(E)
$$
where $\tilde{l}$ is an arbitrary bus in $\calN_l$. $\chi(\calN_l)$ is well-defined by Lemma \ref{lemma:not_directly_connected}. This together with the assumption $\sum_{j\in\calN_l}b_j=0$ then implies
\begin{IEEEeqnarray*}{rCl}
&&\sum_{l\in \calN_l}(-1)^{l+i}b_l\det\paren{\ol{L}^{li}}\\
&=&\sum_{l\in \calN_l}b_l\paren{\sum_{E\in\calT(\set{l,i},\set{z})}\chi(E)}=\sum_{l\in \calN_l}b_l\chi(\calN_l)\\
&=&\chi(\calN_l)\sum_{l\in\calN_l}b_l=0
\end{IEEEeqnarray*}

As a result
\begin{IEEEeqnarray*}{rCl}
&&\sum_{l\notin \calN_1}(-1)^{l+i}b_l\det\paren{\ol{L}^{li}}\\
&=&\sum_{\calN_l\in\calP_1}\sum_{l\in\calN_l}(-1)^{l+i}b_l\det\paren{\ol{L}^{li}}\\
&&+\sum_{\calN_l\in\calP_2}\sum_{l\in\calN_l} (-1)^{l+i}b_l\det\paren{\ol{L}^{li}}\\
&=&\sum_{\calN_l\in\calP_2}\sum_{l\in\calN_l} (-1)^{l+i}b_l\det\paren{\ol{L}^{li}}\\
&=&\sum_{\calN_l\in\calP_2}\sum_{l\in\calN_l}b_l\paren{\sum_{E\in\calT(\set{l,i},\set{z})}\chi(E)}
\end{IEEEeqnarray*}
which by Lemma \ref{lemma:directly_connected} takes the same value for all $i\in\ol{\calN}_1$. In other words, the equation \eqref{eqn:component_inversion} takes the same value for all $i\in\ol{\calN}_1$. This completes the proof. \qed


==> proofs.tex <==
% \section{Proof of Lemma \ref{lemma:zero_branch_deviation}}\label{section:proof_of_zero_branch_deviation}
% \input{zero_bridge_flow_deviation_proof}

% \section{Proof of Proposition \ref{prop:localizability}}\label{section:proof_of_localizability}
% \input{zero_injection_deviation_proof}

\add{\section{Proof of Lemma \ref{lemma:laplace_solvability} \label{section:proof_of_laplace_solvability}}
\input{laplace_solvability_proof}}

% \section{Proof of Proposition \ref{prop:dual_to_infinity}}\label{section:proof_of_blow_up}
% \input{blow_up_proof}
%
%\section{$N-2$ Security}
%\input{n_minus_2}

==> region_separation.tex <==
\section{Region Separation of Power Flows}\label{section:region_separation}
We presented an example in Section \ref{section:critical} demonstrating technical subtleties when speaking of region ``separation'' as an intuitive concept. In this Appendix,

\subsection{Unchanged Tie-Line Flows}
First
\subsection{Unchanged Tie-Line Flows and Unchanged Injections}

==> setup.tex <==
\section{Detailed Simulation Setup}\label{section:setup}

% \begin{figure}[t]
% \centering
% \includegraphics[width=.9\columnwidth]{figs/IEEE118_3_new.pdf}
% \caption{One line diagram of the IEEE 118-bus test network.
% %with three balancing areas. 
% 	%Dashed blue lines are switched off to create a tree-partitioned network with two bridge-blocks. Then dashed green lines are switched off to further partition Area 2 into 2 smaller bridge-blocks. Solid blue and green lines are resulted bridges.
% 	}\label{fig:IEEE_118}
% \end{figure}

The original IEEE 118-bus test network is shown by the solid lines and nodes in Fig.~\ref{fig:IEEE_118}, in which the balancing areas are connected by multiple tie-lines, yielding a trivial bridge-block decomposition with a single bridge-block for the whole network. For our experiments in Section \ref{section:case_study_n_1}, we switch off three lines $(15,33)$, $(19,34)$, and $(23,24)$ to form a tree-partitioned network with two bridge-blocks, shown as Area 1 and Area 2 (which consists of Area 2(a) and Area 2(b)) in the diagram. For our experiments in Section \ref{section:localized_exp}, we further switch off the lines $(77,82)$, $(96,97)$, $(98,100)$, $(99,100)$ to create a tree-partitioned network with three bridge-blocks.

To provide a comprehensive comparison between the proposed control strategy and AGC, we generate \add{several} failure scenarios as summarized in Table~\ref{table:sampling_rate} and simulate the corresponding cascading processes. 
We adopt data from MatPower \cite{zimmerman2011matpower} as the nominal load profile, and add up to 25\% random perturbations to the base value. For $k=1,2,3$ initial line failures, we generate 100, 15, and 15 load profiles and further compute the optimal generation dispatch by DC OPF. For each load profile, we iterate over every single transmission line failure, and sample 3,000 and 5,000 failure scenarios for $k=2,3$ line failures respectively. In total, \add{136,800} failure scenarios are simulated for each control method.

\begin{table}[h]
	\def\arraystretch{1.3}
	\centering{
		\caption{Simulation setup for $N-k$ security evaluation.}\label{table:sampling_rate}
		\begin{tabular}{|c|c|c|c|}
			\hline
			Case & $k=1$ & $k=2$ & $k=3$\\
			\hline
			\# of Load Profiles & 100 & 15 & 15 \\
			\hline
			\# of Sampled Failures & 186 & 3000 & 5000\\
			\hline
			Total Scenarios & 18600 & 45000 & 75000\\
			\hline
		\end{tabular}
	}
\end{table}

==> topology.tex <==
\section{One Line Diagram of IEEE 118-Bus Test Network} \label{section:topology}
%\lguo{Chen: can you help update the diagram to include the switching off to create a third region?}
%The one-line diagram of the IEEE 118-bus test system are shown in Fig.~\ref{fig:IEEE_118}. The system data such as

%\subsection{System Overview and Control Scenarios}

%\begin{subequations}\label{eqn:agc_olc}
%\begin{IEEEeqnarray}{ll}
%\min_{f, d, \theta} \quad& \sum_{j\in\calN}c_j(d_j) \\
%\hspace{.1cm}\text{s.t.} & r - d - Cf = 0 \\
%& f = BC^T\theta \\
%& ECf = 0\\
%& \ul{d}_{j}\le d_j\le \ol{d}_j, j \in\calN
%\end{IEEEeqnarray}
%\end{subequations}

%Both AGC and UC are designed to be \textit{Demand First} for constraint lifting. 
%For AGC, \eqref{eqn:agc_olc} is first solved without allowing any load shedding. If \eqref{eqn:agc_olc} is infeasible, load shedding will then be allowed. AGC is not guaranteed to stop the failures, thus multiple stages might be simulated before the system operates under a secure operating point. We set the maximum simulation stage to be 5 in order to avoid numerical issues. System states at the last simulation stage are recorded no matter whether the system is stable or not. 
%For UC,  \eqref{eqn:uc_olc} is first solved without allowing any load shedding. If necessary, the tie-line constraint will be the first to be lifted, leaving load shedding as the very last action to make the UC optimization problem feasible and stabilize the system. As a consequence, UC will always stop the failure in the first stage, possibly at the cost of some load loss. 

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figs/IEEE118_3_new.pdf}
\caption{One line diagram of the IEEE 118-bus test network.
%with three balancing areas. 
	%Dashed blue lines are switched off to create a tree-partitioned network with two bridge-blocks. Then dashed green lines are switched off to further partition Area 2 into 2 smaller bridge-blocks. Solid blue and green lines are resulted bridges.
	}\label{fig:IEEE_118}
\end{figure}

The original IEEE 118-bus test network is shown by the solid lines and nodes in Fig.~\ref{fig:IEEE_118}, in which the balancing areas are connected by multiple tie-lines, yielding a trivial bridge-block decomposition with a single bridge-block for the whole network. For our experiments in Section \ref{section:case_study_n_1}, we switch off three lines $(15,33)$, $(19,34)$, and $(23,24)$ to form a tree-partitioned network with two bridge-blocks, shown as Area 1 and Area 2 (which consists of Area 2(a) and Area 2(b)) in the diagram. For our experiments in Section \ref{section:localized_exp}, we further switch off the lines $(77,82)$, $(96,97)$, $(98,100)$, $(99,100)$ to create a tree-partitioned network with three bridge-blocks.
